HighLight: Efficient and Flexible DNN Acceleration with Hierarchical Structured Sparsity

Due to complex interactions among various deep neural network (DNN) optimization techniques, modern DNNs can have weights and activations that are dense or sparse with diverse sparsity degrees. To offer a good trade-off between accuracy and hardware performance, an ideal DNN accelerator should have high flexibility to efficiently translate DNN sparsity into reductions in energy and/or latency without incurring significant complexity overhead. This paper introduces hierarchical structured sparsity (HSS), with the key insight that we can systematically represent diverse sparsity degrees by having them hierarchically composed from multiple simple sparsity patterns. As a result, HSS simplifies the underlying hardware since it only needs to support simple sparsity patterns; this significantly reduces the sparsity acceleration overhead, which improves efficiency. Motivated by such opportunities, we propose a simultaneously efficient and flexible accelerator, named HighLight, to accelerate DNNs that have diverse sparsity degrees (including dense). Due to the flexibility of HSS, different HSS patterns can be introduced to DNNs to meet different applications' accuracy requirements. Compared to existing works, HighLight achieves a geomean of up to 6.4x better energy-delay product (EDP) across workloads with diverse sparsity degrees, and always sits on the EDP-accuracy Pareto frontier for representative DNNs

==> 07_hss_pruning.tex <==

\section{DNNs with HSS Patterns}
\label{sec:hss-pruning}
To generate appropriate DNNs for \designName, we prune DNNs with diverse sparsity degrees with various HSS patterns. Since a good set of sparsity patterns should allow reasonable accuracy recovery even without novel or advanced pruning algorithms (\eg, special ways to perform hyper-parameter searches), we reuse the pruning algorithm proposed for sparse tensor core (STC)~\cite{NM-finetune} to demonstrate the easily recoverable nature of HSS-based pruning.

The algorithm for STC first statically prunes a pre-trained dense DNN by masking the appropriate weights and their gradients to zeros, and fine-tunes the masked DNN to regain accuracy. Instead of introducing the 2:4 structure only, which is the structure that can be accelerated by STC, we introduce various HSS patterns to the pre-trained dense DNN. To ensure the weights with larger magnitudes are preserved as much as possible, we prune the weights rank-by-rank in a lower-to-higher fashion. For example, for a C$\textsubscript{1}$(3:4)$\rightarrow$C$\textsubscript{0}$(2:4) HSS, we first apply the rank C$\textsubscript{0}$'s 2:4 structure and then rank C$\textsubscript{1}$'s 3:4 structure. For the lowest rank, we replace the weights with the smallest magnitude with zero. For an intermediate rank, we prune coordinates whose fiber payload has the smallest \emph{scaled L2 norm}, defined as the average magnitude of all weights in the payload. The masked weights and corresponding gradients are kept as zeros and fine-tuning is then performed to update the nonzero weights to regain DNN accuracy. 

%Like prior works~\cite{NM-finetune, NM-permutation}, our experiments (Sec.\ref{sec:pareto}) show that using the same hyperparameters that are used to obtain the trained model can help the fine-tuning process to regain a reasonable amount of accuracy.  
 
 %We note that full retraining is not always necessary and that further training time optimizations are possible (\eg, ~\cite{NM-finetune, learning-rate-rewinding}).


%To generate dual-side sparse workloads, HSS patterns can be applied to activations by dynamically setting activations (and their gradients) to zero for each mini-batch~\cite{NM_iact_pruning, DASNet-iact-pruning, s2ta}. 


